Learning the Predictability of the Future

We introduce a framework for learning from unlabeled video what is predictable in the future. Instead of committing up front to features to predict, our approach learns from data which features are predictable. Based on the observation that hyperbolic geometry naturally and compactly encodes hierarchical structure, we propose a predictive model in hyperbolic space. When the model is most confident, it will predict at a concrete level of the hierarchy, but when the model is not confident, it learns to automatically select a higher level of abstraction. Experiments on two established datasets show the key role of hierarchical representations for action prediction. Although our representation is trained with unlabeled video, visualizations show that action hierarchies emerge in the representation.

==> figures/results_earlyaction_hollywood2.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.15,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={\#participants},
    symbolic x coords={tool8,tool9,tool10},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {(tool8,7) (tool9,9) (tool10,4)};
\addplot coordinates {(tool8,4) (tool9,4) (tool10,4)};
\addplot coordinates {(tool8,1) (tool9,1) (tool10,1)};
\legend{used,understood,not understood}
\end{axis}
\end{tikzpicture}

==> old_method.tex <==
\section{Method}

%I felt pretty thrown by the first paragraph of this section. I had a nice introduction in section 1 to what you want to do and the motivation and an interesting related work section, now I expected your to start explaining your method, but instead I get a detailed explanation of how DPC works. Reading through this for the first time I don’t really get where this is going. Can you add an opening paragraph that charts the journey you’re going to take me through in this section? I’m just skimming through the rest of section 3 to see what you’re going to talk about, it looks like you’re using DPC with a hyperbolic space. The first paragraph doesn’t state you’re going to use DPC so at this point I’m unsure how the information you’re giving me is relevant to your paper. 
%I think you need to:
%1. Change opening paragraph of sec 3 to explain that you use DPC rather than saying “we follow the formulation in [11]”, does that mean loss function? model architecture? I don’t know until I read the rest of this section.
%2. Give me a bit of a guide to what you’re going to explain in all of sec 3 before we dive into sec. 3.1 
%3. Give me a little summary at the top of sec 3.1 about what you’re going to cover in this subsection, I don’t think 3.2/3.3/3.4 need that as the titles make it obvious what you’re going to cover.

We introduce a self-supervised framework to learn video representations that implicitly deals with the variable predictability of the future, and that is capable of selecting the appropriate abstraction level based on the available information. We use DPC \cite{han2019video}, with the simple but key difference of operating in the hyperbolic space instead of the Euclidean one. The motivation for this change comes from the geometric properties of the hyperbolic space, that naturally encodes hierarchical structures. Following the motivation presented in the introduction, our loss function implicitly encourages the model to predict specific concepts when it is confident and abstract ones when it is not.

\begin{figure}
\includegraphics[width=\linewidth]{figures/poincare_ball.pdf}
\caption{The future is non-deterministic. Given a specific past (first three frames in the figure), different representations (represented by crosses in the Poincar\'e ball) can encode different futures, all of them possible. In case the model is uncertain, it will predict an abstration of all these possible futures, represented by the $x$. The more confident it is, the more specific the prediction can get. Assuming the actual future is represented by $y$, the gray arrows represent the trajectory the prediction will follow as more information is available.}
\label{fig:poincare_ball}
\end{figure}

The rest of this section is structured as follows. In Section~\ref{sec:learning} we explain DPC and the only change we make to it, which is changing the geometric space from Euclidean to hyperbolic. \ds{Write better, but it has to be easy for the reader to follow}. Section~\ref{sec:model} describes the used architecture, in Section~\ref{sec:classification} we explain how we test the representation on labeled data, and finally we provide more details about the implementation in Section~\ref{sec:implementation}.

\subsection{Learning hyperbolic video representations}
\label{sec:learning}

\ds{This subsection is too long. We either split it, or move something to the intro of the section}


\cv{I would write this section independent of DPC. You can frame this as wanting to learn features, and you adopt a contrastive approach. Give the contrastive objective first. Highlight the challenges with the contrastive objective for prediction -- that it does not encode uncertainty, and instead discards it. Before you end this section, you can mention how many different approaches use contrastive objectives, DPC is one of them, but you can also mention SimCLR. Then, in the next subsection, talk about the distance metric.}

\cv{I think if you write it this way, it will highlight the fundamental contribution and not seem incremental to DPC}

In this section we first introduce DPC \cite{han2019video}, and then explain how our method uses DPC with the single but crucial change of modifying the geometric space where the distances are computed.

%Idea 1 in this section: Video representations with contrastive learning. Quickly explain what contrastive learning is, that we use contrastive learning to predict into the future, etc.
The spatial and temporal consistency in videos make it a rich signal to learn self-supervised representations. Contrastive learning frameworks have been proposed \cite{han2019video} that formulate the learning as a proxy task that predicts representations of future frames given past ones. They create views of individual videos at different spatio-temporal locations and pose the learning in a contrastive setting in which negatives are selected by sampling the correct spatial position at incorrect temporal steps or vice versa, as well as sampling the negatives from different videos in a mini batch. In our paper, we adopt the exact same formulation. 

In order to provide a score for a pair or video representations, a similarity measure is required. In the contrastive learning literature, this is usually a cosine similarity, which is equivalent to the negative of the squared Euclidean L2 distance when the representations are normalized to have norm $1$.\footnote{$||a-b||^2_2=a^Ta+b^Tb-2a^Tb \stackrel{*}{=}2-2d_{\text{cos}}(a, b)$, where $\stackrel{*}{=}$ denotes an equality based on the fact that the representations are normalized to have norm $1$. The first $2$ is cancelled out in the contrastive loss, and the $2$ that is multiplying gets absorbed into the $\tau$.}

% Idea 2: But there is uncertainty. Our main idea is SIMPLE: change space from euclidean to hyperbolic. This implies changing the distance metric. Here explain some maths of hyperbolic space, and end up with the equation of the distance.
The future of videos, however, is intrinsically non-deterministic. The previous framework can overcome this problem by generating features that are invariant to all possible futures (given some past information), and thus creating a general representation for all of them. Nevertheless, this does not account for the variability of the required abstraction, where some predictions can be more specific than others: the geometry of the Euclidean space cannot reflect such a structure.

The key contribution of this paper lies on the simple idea of changing the representation space to work in a space that naturally handles the uncertainty of the predictions. Specifically, we propose encoding video representations in the hyperbolic space, which is naturally suited to encode hierarchies \cite{Gromov1987HyperbolicG}. Thus, the representation will be able to move from more abstract concepts in case of low predictability, to specific ones in case the future is clear. In practice, this has the main requirement of changing the distance metric.

The hyperbolic $n$-space, or $\mathbb{H}^n$, is one of the three isotropic model spaces of the Riemannian geometry, defined by having constant negative curvature.\footnote{In this paper we assume the curvature to be $-1$.}\textsuperscript{,}\footnote{The other two spaces are the Euclidean space $\mathbb{R}^n$ (zero curvature), and the spherical space $\mathbb{S}^n$ (constant positive curvature).} 
The hyperbolic space has five isometric models, and the Poincar\'e model is the most used in the deep learning literature. The \textit{Poincar\'e ball model} is defined by the manifold $\mathbb{D}^n = \{X\in\mathbb{R}^n : ||x|| < 1\}$ and the Riemmanian metric $g^\mathbb{D}$:
 
\begin{equation}
  g_{x}^{\mathbb{D}}=\lambda_{x}^{2} g^{E}, \quad \text { where } \lambda_{x}:=\frac{2}{1-\|x\|^{2}},
  \label{eq:metric}
\end{equation}

where $g^E=\textbf{I}_n$ is the Euclidean metric tensor. The distance induced by this metric in the manifold $\mathbb{D}^n$ has the following form:

\begin{equation}
    d_{\mathbb{D}}(x, y)=\cosh ^{-1}\left(1+2 \frac{\|x-y\|^{2}}{\left(1-\|x\|^{2}\right)\left(1-\|y\|^{2}\right)}\right).
    \label{eq:distance}
\end{equation}

% Now explain some intuition
\ds{This paragraph should be centered around \ref{fig:poincare_ball}}
This is the distance we use in our framework. When computing graph distances in trees, the mean point (in terms of sum of squared distances) between two leaf nodes is not another leaf node, but a node that is higher in the hierarchy. Therefore, in case the prediction between the two leaf nodes is not possible given the provided information, the expected squared distance will be minimized by selecting the more abstract one as the prediction, the same way we would predict ``greeting'' when we doubt between ``handshake'' or ``high five'' in Fig.~\ref{fig:teaser}. The Poincar\'e ball, represented in Fig.~\ref{fig:poincare_ball}, is similar: points closer to the edge of the ball represent more specific concepts and can be related to the lower level nodes in a tree. Points closer to the center of the Poincar\'e ball represent more abstract concepts, that encompass the specific ones. In this case, the mean point between two points close to the edge of the ball --exemplified by the top two crosses in Fig.~\ref{fig:poincare_ball}-- is not another node at the same level, but a node further from the edge, represented with a pink circle. The line connecting the two crosses is the minimum distance path between them, and is called a \textit{geodesic}. It is worth noting that the hyperbolic space is, unlike trees, continuous, and as such there is not a defined number of hierarchy levels, but a continuum from very specific (closer to the border of the Poincar\'e ball) to very abstract (closer to the center).

% Idea 3: Finally, this is the loss (equation of the contrastive loss). Does not have to be super specific (eg we still havenn't described the networks g and f)
Once the distance is defined, the contrastive loss can be directly adapted from \cite{han2019video}, where we change the similarity function to be defined by the hyperbolic metric instead of Euclidean one:

\begin{equation}
    \mathcal{L}=-\sum_{i}\left[\log \frac{\exp \left(-d^2_{\mathbb{D}}({{}\hat{z}_\mathbb{D}}_i, {z_\mathbb{D}}_{i})\right)}{\sum_{j} \exp \left(-d^2_{\mathbb{D}}({{}\hat{z}_\mathbb{D}}_i, {z_\mathbb{D}}_{j})\right)}\right]
    \label{eq:loss}
\end{equation}
% Two alternatives, with and without parenthesis
% \mathcal{L}=-\sum_{i}\left[\log \frac{\exp \left(-d_{\mathbb{D}}({{}\hat{z}_\mathbb{D}}_i, {z_\mathbb{D}}_{i})\right)}{\sum_{j} \exp \left(-d_{\mathbb{D}}({{}\hat{z}_\mathbb{D}}_i, {z_\mathbb{D}}_{j})\right)}\right]
% \mathcal{L}=-\sum_{i}\left[\log \frac{\exp \left(-d_{\mathbb{D}}((\hat{z}_\mathbb{D})_i, (z_\mathbb{D})_{i})\right)}{\sum_{j} \exp \left(-d_{\mathbb{D}}( (\hat{z}_\mathbb{D})_i, (z_\mathbb{D})_{j})\right)}\right]

where $z_\mathbb{D}$ is the feature representing a spatio-temporal location in a video, and $\hat{z_\mathbb{D}}$ is the prediction of that feature. %We maintain the the square of the distance, as it is used in the original formulation. 
Importantly, the representations $z_\mathbb{D}$ have to be in the Poincar\'e ball. Features with index $j\neq i$ are negatives that define the distribution of distances between predictions $\hat{z_\mathbb{D}}$ and features $z_\mathbb{D}$. Then the positive pairs (where the indices of the prediction and the feature is the same) are contrasted to this distribution. These negatives are obtained by using features from other clips in the mini batch, as well as using features that correspond to the same clip but in incorrect spatial or temporal locations.

\subsection{Model}
\label{sec:model}


\begin{figure}
  \includegraphics[width=\linewidth]{figures/architecture.pdf}
  \caption{Architecture of our method. Blue and red represent Euclidean and hyperbolic layers and representations, respectively.}
  \label{fig:architecture}
\end{figure}
% \ds{This is details about the previous paragraph}

% Here we explain networks g and f, the overall way of creating both temporal, spatial and inter-batch negatives, etc. 
We show a general overview of the model in Fig.~\ref{fig:architecture}. A video clip is partitioned into subclips $x_t\in\mathbb{R}^{T\times H\times W\times 3}$ (time $\times$ height $\times$ width $\times$ channels) of equal length, each one representing a time step $t$. An encoder network $f(.)$ takes each subclip as input, and generates a latent representation $z_t\in\mathbb{R}^{1\times H'\times W'\times C}$. Note that $z_t$ preserves spatial information ($H'>1$ and $W'>1$). Context representations $c_t$ at each time step are obtained by temporally aggregating representations $z$ with a function $g(.)$. Finally, this contextual information is used to predict the future representations $\hat{z}$ using the prediction network $\phi(.)$. In some of our experiments we allow $\phi(.)$ to predict $n$ steps into the future, in which case $n$ is an input to $\phi(.)$ as well:

\begin{align}
  z_t = f(x_t) \\
  c_t = g(z_1, z_2, \dots, z_t) 
  \label{eq:ct} \\
  \hat{z}_{t+n} = \phi(c_t, n)
  \label{eq:phi}
\end{align}

In an autoregressive setting, the last $z_t$ in Eq.~\ref{eq:ct} can be replaced by predictions $\hat{z}_t$. Unless otherwise noted, we use the same parameters as in \cite{han2019video} -- refer to that paper for more details. % use "maps"

We add one crucial extension to the presented model, which consists in projecting representations to the hyperbolic space.
The transition from the Euclidean space is based on the process mapping to Riemannian manifolds from their corresponding tangent spaces. A \textit{Riemnnian manifold} is a pair ($\mathcal{M}$, $g$), where $\mathcal{M}$ is a smooth manifold and $g$ is a Riemmanian metric, such as the presented in Eq.~\ref{eq:metric}. Broadly, smooth manifolds are spaces that locally look like some Euclidean space $\mathbb{R}^n$, and on which one can do calculus \cite{lee2013smooth}, and this is precisely the connection between the two spaces. For $x \in \mathcal{M}$, one can define the tangent space $T_x\mathcal{M}$ of $\mathcal{M}$ at $x$ as the first order linear approximation of $\mathcal{M}$ around $x$. 

The \textit{exponential map} $\text{exp}_x: T_x\mathcal{M}\rightarrow \mathcal{M}$ at $x$ is a map from the tangent spaces into the manifold: it gives a way to project back a vector $v$ of the tangent space $T_x\mathcal{M}$ at $x$, to a point $\text{exp}_x(v) \in\mathcal{M} $ on the manifold. The exponential map is important to project back results of operations in the tangent space to the manifold, like for example when performing gradient updates \cite{Bonnabel2013}. The inverse of the exponential map is called \textit{logarithmic map} and denoted $\text{log}_x$. 

Following \cite{Liu2020}, we use an exponential map centered at $\textbf{0}$ to project from the Euclidean space to the hyperbolic space. Once the representations are in the hyperbolic space, the mathematical operations and the optimization follow the rules derived by the metric in that space: Riemmanian metrics allow us to define lengths, angles, and distances on smooth manifolds. Essentially, they define an inner product on each tangent space $T_x\mathcal{M}$ of the manifold, such that the inner products $g_x : T_x\mathcal{M}\times T_x\mathcal{M} \rightarrow \mathbb{R}$ vary smoothly with $x$ \cite{lee2013smooth}.  Having defined a collection of local inner products $g_x$, a global distance function $d: \mathcal{M} \times \mathcal{M}\rightarrow \mathbb{R}_+$ can be defined to be the infimum of the lengths of all curves from $x$ to $y$ \cite{lee2006riemannian}:
\begin{equation}
    d(x, y)=\inf _{\gamma} L_g(\gamma),
\end{equation}

where $\gamma: [a, b] \rightarrow \mathcal{M}$ is a curve, and $L_g(\gamma)$ is the length of the curve, defined as:
\begin{equation}
    L_g(\gamma)=\int_{a}^{b}|\dot{\gamma}(t)| d t = \int_{a}^{b} \sqrt{g_{\gamma(t)}(\dot{\gamma}(t), \dot{\gamma}(t))} d t.
\end{equation}

In the specific case of the Poincar\'e ball model, this distance is the one in Eq.~\ref{eq:distance}. Based on these concepts, several papers define extensions of the standard (Euclidean) neural network layers to the hyperbolic geometry \cite{Ganea2018,shimizu2020hyperbolic,Chami2019,Liu2019b,Gulcehre2019}. We use the hyperbolic feed-forward layer defined in \cite{Ganea2018} to obtain the representation $z_\mathbb{D}$ that we use in Eq.~\ref{eq:loss}, from the Euclidean representation $z$.
Specifically, we apply this layer after the exponential map, as shown in Fig~\ref{fig:architecture}.

\subsection{Classification}
\label{sec:classification}

Once our model has been trained, we train a linear layer on top of the representations in a supervised way, while freezing the rest of the model. When the representation is hyperbolic, instead of using an Euclidean linear layer, we use the multiclass logistic regression layer from \cite{Ganea2018}, that assumes the input representations are in the Poincar\'e ball, and learns hyperplanes in the same space.

\subsection{Implementation details}
\label{sec:implementation}

Following \cite{han2019video}, $f(.)$ is implemented as a 3D-ResNet18, and $g(.)$ consists of a one-layer Convolutional Gated Recurrent Unit (ConvGRU) with kernel size $(1,1)$. $\phi(.)$ is implemented using a two-layer perceptron.

In order to select subclips, in general we just subsample $N$ non overlapping blocks from the original video clip, consisting of $T$ frames each. In cases where divisions into subclips are given by the dataset, we use those as inputs. % Give more details about which frames are selected.

% To optimize the system we use Riemannian Adam \cite{becigneul2018riemannian} that takes into account the geometry \ref{eq:metric}. We use the Geoopt library in Pytorch \cite{geoopt2020kochurov,pytorch}.

% \ds{Basile: perhaps it is worth nothing the dimensionality of videos and networks here, since they are not noted anywhere else. + how about numberof epochs, learning rate etc. ?}

\vfill\pagebreak
